Towards Causal Deep Learning for Vulnerability Detection

Deep learning vulnerability detection has shown promising results in recent years. However, an important challenge that still blocks it from being very useful in practice is that the model is not robust under perturbation and it cannot generalize well over the out-of-distribution (OOD) data, e.g., applying a trained model to unseen projects in real world. We hypothesize that this is because the model learned non-robust features, e.g., variable names, that have spurious correlations with labels. When the perturbed and OOD datasets no longer have the same spurious features, the model prediction fails. To address the challenge, in this paper, we introduced causality into deep learning vulnerability detection. Our approach CausalVul consists of two phases. First, we designed novel perturbations to discover spurious features that the model may use to make predictions. Second, we applied the causal learning algorithms, specifically, do-calculus, on top of existing deep learning models to systematically remove the use of spurious features and thus promote causal based prediction. Our results show that CausalVul consistently improved the model accuracy, robustness and OOD performance for all the state-of-the-art models and datasets we experimented. To the best of our knowledge, this is the first work that introduces do calculus based causal learning to software engineering models and shows it's indeed useful for improving the model accuracy, robustness and generalization. Our replication package is located at https://figshare.com/s/0ffda320dcb96c249ef2.

==> body/5.results.bck.tex <==
\section{Results}
\label{sec:results}
\subsection{RQ1: Model Accuracy}


\begin{table}[t]
\setlength{\tabcolsep}{2pt}
\caption{ The F1 score of \tool{} and the vanilla model on the test set of Devign and Big-Vul dataset. }
\begin{tabular}{l|cc|cc|cc}
\toprule
Settings  & \multicolumn{2}{c|}{CodeBERT}        & \multicolumn{2}{c|}{GraphCodeBERT}   & \multicolumn{2}{c}{UniXcoder}       \\ \midrule
          & \multicolumn{1}{c|}{Devign} & Big-Vul    & \multicolumn{1}{c|}{Devign} & Big-Vul    & \multicolumn{1}{c|}{Devign} & Big-Vul    \\ \midrule
Vanilla   & \multicolumn{1}{c|}{0.61} & 0.38 & \multicolumn{1}{c|}{0.63} & 0.38 & \multicolumn{1}{c|}{0.64} & 0.39 \\ \midrule
Var1      & \multicolumn{1}{c|}{0.65} & 0.40 & \multicolumn{1}{c|}{0.63} & 0.38 & \multicolumn{1}{c|}{0.66} & 0.40 \\ 
Var2      & \multicolumn{1}{c|}{0.64} & 0.40 & \multicolumn{1}{c|}{0.63} & 0.40 & \multicolumn{1}{c|}{0.65} & \textbf{0.41} \\ 
% Var3      & \multicolumn{1}{c|}{0.63} & 0.40 & \multicolumn{1}{c|}{0.61} & 0.40 & \multicolumn{1}{c|}{0.64} & 0.39 \\ 
\midrule
API1      & \multicolumn{1}{c|}{0.63} & 0.40 & \multicolumn{1}{c|}{0.62} & \textbf{0.41} & \multicolumn{1}{c|}{0.64} & 0.40 \\ 

API2      & \multicolumn{1}{c|}{0.65} & 0.40 & \multicolumn{1}{c|}{0.64} & 0.40 & \multicolumn{1}{c|}{0.66} & 0.40 \\ 
API3      & \multicolumn{1}{c|}{\textbf{0.66}} & 0.40 & \multicolumn{1}{c|}{0.65} & 0.38 & \multicolumn{1}{c|}{\textbf{0.68}} & 0.40 \\ 
\midrule
Var+API & \multicolumn{1}{c|}{0.65} &\textbf{0.41} & \multicolumn{1}{c|}{\textbf{0.66}} & 0.39 & \multicolumn{1}{c|}{0.66} & 0.40 \\ 
\bottomrule
\end{tabular}
\label{tab: rq1}
\end{table}
% \textbf{Baselines}: We compare the performance  of  our causal approach with three state-of-art transformer-based deep learning models: CodeBERT, UniXcoder and GraphCodeBERT. We select these models because their pretrained model is widely used for downstream tasks like vulnerability detection. We address these models as the "Vanilla" models in our work.

% \textbf{Result:} 
Table~\ref{tab: rq1} shows that \tool{} outperform  the vanilla models for all the settings, all the datasets and all the models.

For Devign data, \tool{} Var1~\ray{what are these?}, API3, and VAR+API show 4\%, 5\%, and 4\%  improvement respectively in terms of the F1-score against the CodeBERT vanilla model. In the UniXcoder models, the improvement for these three approaches are 2\%, 4\% and 2\% respectively. With the GraphCodeBERT model, our approaches API3 and Var+API show 2\% and 3\% improvement against the vanilla model. Overall, our approaches show 2-5\%  f1 score improvement against the vanilla model. We can see that Var1 and API3 settings show constant improvement with the three models.

For the Big-Vul dataset, our causal approaches with the CodeBERT model show a 2-3\% improvement, so do the GraphCodeBERT and UniXcoder models.

%Our approaches with the other two models e.g. GraphCodeBERT and UniXcoder show a similar trend. Overall, our causal approach outperforms the vanilla models.

\subsection{RQ2: Model Robustness and Generalization}
\wei{It is showing due to the causal effect, the probability distribution of the vulnerable samples move more towards vulnerable probability}

\textbf{Robustness:} Table \ref{tab:robustness_table} shows the robustness performance. There are three blocks of the table. The upper block presents the result where our Causal Name settings and the vanilla models are evaluated on the worst perturbVar data. In the middle block, the Causal API settings and the vanilla models are evaluated on the worst PerturbAPI data. The last block compares the performance of the Causal Combined settings against the vanilla model by evaluating the worst PerturbJoint data. Our Causal Name settings show at most 6\%, 3\% and 2\% improvement with CodeBERT, GraphCodeBERT and UniXcoder model respectively for the Devign data. While in Big-Vul data, the improvement is 1\%, 4\% and 4\% respectively. Overall, our Causal Name approach works better than the vanilla model in terms of robustness.   For Devign data, the Causal API settings demonstrate at most 10\%, 5\% and 22\% improvement with the three models respectively. For the Big-Vul data, the improvement is 3\%, 2\% and 5\% respectively respectively.
Our Causal combined settings show similar trends.
% \begin{table}[!ht]
%     \centering
%     \begin{tabular}{|l|l|l|l|l|l|}
%         \toprule
%         Causal Setting & CodeBERT + Devign & CodeBERT + Big-Vul & GraphCodeBERT + Devign & GraphCodeBERT + Big-Vul & UniXcoder + Devign \\ 
%         \midrule
%         var & trivial & midium & trivial & small & trivial \\ \hline
%         api & large & midium & small & small & large \\ \hline
%         combine & large & small & large & small & small \\ 
%         \bottomrule
%     \end{tabular}
% \end{table}
\rasel{
In figure \ref{fig:probability_density_vul}, predicted probability density for the Devign vulnerable data. In each subplot, X-axis is the predicted probability of being vulnerable and  Y-axis is the count of the examples whose predictions are that probability. The plot demonstrates that the overall prediction probability for vulnerable data is increasing.  We also do the statistically significant test and the result shows that they are statistically significant with $P<<<0.05.$
}
Overall, our causal approaches outperform vanilla models in terms of robustness.
\begin{table}[]
\caption{The Robustness performance of \tool{} and the vanilla models}
\setlength{\tabcolsep}{2pt}
\begin{tabular}{l|cc|cc|cc}
\toprule
Settings  & \multicolumn{2}{c|}{CodeBERT}                          & \multicolumn{2}{c|}{GraphCodeBERT}                     & \multicolumn{2}{c}{UniXcoder}                         \\ \midrule
          & \multicolumn{1}{c|}{Devign} & \multicolumn{1}{c|}{Big-Vul} & \multicolumn{1}{c|}{Devign} & \multicolumn{1}{c|}{Big-Vul} & \multicolumn{1}{c|}{Devign} & \multicolumn{1}{c}{Big-Vul} \\ \midrule
Vanilla   & \multicolumn{1}{c|}{0.52}   & 0.22                     & \multicolumn{1}{c|}{0.58}   & 0.26                     & \multicolumn{1}{c|}{0.52}   & 0.19                     \\\hline
Var1      & \multicolumn{1}{c|}{\textbf{0.58}}   & \textbf{0.23}                     & \multicolumn{1}{c|}{\textbf{0.61}}   & 0.28                     & \multicolumn{1}{c|}{\textbf{0.54}}   & 0.21                     \\ 
Var2      & \multicolumn{1}{c|}{0.55}   & 0.22                     & \multicolumn{1}{c|}{0.58}   & {\bf 0.30}                     & \multicolumn{1}{c|}{0.53}   & 0.22                     \\\hline
% Var3      & \multicolumn{1}{c|}{0.56}   & 0.22                     & \multicolumn{1}{c|}{0.59}   & \textbf{0.30}                     & \multicolumn{1}{c|}{0.53}   & \textbf{0.23}                     \\ 
\midrule
Vanilla   & \multicolumn{1}{c|}{0.52}   & 0.10                     & \multicolumn{1}{c|}{0.47}   & 0.09                     & \multicolumn{1}{c|}{0.35}   & 0.09                     \\\hline
API1      & \multicolumn{1}{c|}{0.52}   & 0.13                     & \multicolumn{1}{c|}{0.35}   & \textbf{0.11}                     & \multicolumn{1}{c|}{0.45}   & \textbf{0.14}                     \\ 
API2      & \multicolumn{1}{c|}{0.56}   & \textbf{0.13}                     & \multicolumn{1}{c|}{0.39}   & \textbf{0.11}                     & \multicolumn{1}{c|}{0.49}   & 0.13                    
                    \\\hline
API3      & \multicolumn{1}{c|}{\textbf{0.62}}   & 0.10                     & \multicolumn{1}{c|}{\textbf{0.52}}   & 0.09                     & \multicolumn{1}{c|}{\textbf{0.57}}   & 0.13  \\\hline
 \midrule
Vanilla   & \multicolumn{1}{c|}{0.52}   & 0.06                     & \multicolumn{1}{c|}{0.45}   & 0.07                     & \multicolumn{1}{c|}{0.22}   & 0.05                     \\ 
Var+API & \multicolumn{1}{c|}{\textbf{0.55}}   & \textbf{0.07}                     & \multicolumn{1}{c|}{\textbf{0.54}}   & \textbf{0.08}                     & \multicolumn{1}{c|}{\textbf{0.31}}   & \textbf{0.10}                     \\ 
\bottomrule
\end{tabular}
\label{tab:robustness_table}
\end{table}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/representation_density_1_Devign.png}
\caption{Prediction Probability Density}
\label{fig:probability_density_vul}
\end{figure}

\begin{table}[]
\setlength{\tabcolsep}{2pt}
\caption{The generalization performance of \tool{} and the vanilla models}.
\label{tab:generalization}
\begin{tabular}{l|cc|cc|cc}
\toprule
Settings                          & \multicolumn{2}{c|}{CodeBERT}      & \multicolumn{2}{c|}{GraphCodeBERT} & \multicolumn{2}{c}{UniXcoder}     \\\midrule
\cellcolor[HTML]{FFFFFF}          & \multicolumn{1}{c|}{Devign} & Big-Vul  & \multicolumn{1}{c|}{Devign} & Big-Vul  & \multicolumn{1}{c|}{Devign} & Big-Vul  \\ \midrule
\cellcolor[HTML]{FFFFFF}Vanilla   & \multicolumn{1}{c|}{0.11}   & 0.08 & \multicolumn{1}{c|}{0.11}   & 0.10 & \multicolumn{1}{c|}{0.10}   & 0.07 \\ \midrule
\cellcolor[HTML]{FFFFFF}Var1      & \multicolumn{1}{c|}{0.12}   & 0.17 & \multicolumn{1}{c|}{0.11}   & 0.11 & \multicolumn{1}{c|}{\textbf{0.12}}   & 0.13 \\ 
\cellcolor[HTML]{FFFFFF}Var2      & \multicolumn{1}{c|}{0.12}   & \textbf{0.18} & \multicolumn{1}{c|}{0.11}   & \textbf{0.14} & \multicolumn{1}{c|}{\textbf{0.12}}   & 0.15 \\ 
% \cellcolor[HTML]{FFFFFF}Var3      & \multicolumn{1}{c|}{0.12}   & 0.17 & \multicolumn{1}{c|}{0.11}   & 0.10 & \multicolumn{1}{c|}{0.11}   & 0.13 \\ 
\midrule
\cellcolor[HTML]{FFFFFF}API1      & \multicolumn{1}{c|}{0.12}   & 0.17 & \multicolumn{1}{c|}{0.11}   & 0.12 & \multicolumn{1}{c|}{\textbf{0.12}}   & 0.11 \\ 

\cellcolor[HTML]{FFFFFF}API2      & \multicolumn{1}{c|}{0.12}   & 0.16 & \multicolumn{1}{c|}{0.11}   & \textbf{0.14} & \multicolumn{1}{c|}{\textbf{0.12}}   & 0.18 \\ 
\cellcolor[HTML]{FFFFFF}API3      & \multicolumn{1}{c|}{\textbf{0.13}}   & 0.15 & \multicolumn{1}{c|}{0.11}   & 0.10 & \multicolumn{1}{c|}{\textbf{0.12}}   & \textbf{0.21} \\
 \midrule
\cellcolor[HTML]{FFFFFF}Var+API & \multicolumn{1}{c|}{0.12}   & 0.17 & \multicolumn{1}{c|}{0.11}   & 0.12 & \multicolumn{1}{c|}{\textbf{0.12}}   & 0.18 \\ 
\bottomrule
\end{tabular}
\end{table}


\textbf{Generalization:} We present the generalization results in Table \ref{tab:generalization}. The Devign column defines the f1 score of the Big-Vul test set when evaluated on the model trained with the Devign train set. Similarly, the Big-Vul column presents the f1 score of the Devign test set evaluated on the model that is trained with the Big-Vul train set. When the model is trained on the Devign train set and the Big-Vul test set is used as the OOD, our causal approach shows 1\%-2\% improvement for CodeBERT and UniXcoder models.   But when the Devign test set is used as the OOD data on the model trained with Big-Vul data, CodeBERT model shows 7-10\% improvement, GraphCodeBERT model shows at most 4\% improvement and UniXcoder model shows 6-14\% improvement. Overall,  our causal approach works better with the  OOD data.



%\subsection{RQ3: Interpreting Models}
% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.48\textwidth]{figures/representation_density_1.pdf}
% \caption{Prediction Probability Density}
% \label{fig:interpretation-analysis-results}
% \end{figure}
\subsection{RQ3: Ablation Studies}

\rasel{
In figure \ref{fig:prob_k_1vs40}, we present the result of the ablation studies using K=1. In each subplot, X-axis is the predicted probability of being vulnerable and  Y-axis is the count of the examples whose predictions are that probability. From the result, we can see that for the vulnerable examples, the probabilities are nearer to 1.0 while K=40 is used than K=1. Similarly, for the non-vulnerable examples, the probabilities are nearer to 0.0 while K=40 is used than K=1. Though the GraphCodeBERT model with vulnerable data shows some different result, but if we consider the local pick before probability 0.50 which is lower with K = 40 than K=1, it is clear that K=40 is better than K=1. Because of space, we only show the performance on Devign data.


% the \tool approach with the CodeBERT model shows 4\% and 2\% improvement respectively, however, the improvement was 5\% and 3 \% respectively with K=40.

}
% We can see a similar trend for GraphCodeBERT and UniXcoder models. Overall, the \tool approach can reduce the impact of spurious features but not like the marginalization with K=40.


% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.45\textwidth]{figures/codebert_devign_early_layer.pdf}
% \caption{Ablation studies on passing $X'$ through first nth encoder block of the transformer models.
% }
% \label{fig:interpretation-analysis-results}
% \end{figure}
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \begin{table}[]
% \setlength{\tabcolsep}{2pt}
% \caption{The f1 score of the vanilla model and \tool{} when K=1}
% \begin{tabular}{l|cc|cc|cc}
% \toprule
% Settings  & \multicolumn{2}{c|}{CodeBERT}         & \multicolumn{2}{c|}{GraphCodeBERT}    & \multicolumn{2}{c}{UniXcoder}        \\ \hline
%           & \multicolumn{1}{c|}{Devign} & Big-Vul & \multicolumn{1}{c|}{Devign} & Big-Vul & \multicolumn{1}{c|}{Devign} & Big-Vul \\ \hline
% Vanilla   & \multicolumn{1}{c|}{0.61}   & 0.38    & \multicolumn{1}{c|}{0.63}   & 0.38    & \multicolumn{1}{c|}{0.64}   & 0.39    \\ 
% Var1      & \multicolumn{1}{c|}{0.64}   & 0.39    & \multicolumn{1}{c|}{0.64}   & 0.38    & \multicolumn{1}{c|}{0.65}   & \textbf{0.41}    \\ 
% Var2      & \multicolumn{1}{c|}{0.64}   & 0.39    & \multicolumn{1}{c|}{0.63}   & 0.39    & \multicolumn{1}{c|}{0.65}   & 0.40    \\ 
% \midrule
% API1      & \multicolumn{1}{c|}{0.63}   & \textbf{0.40}    & \multicolumn{1}{c|}{0.62}   & \textbf{0.41}    & \multicolumn{1}{c|}{0.64}   & 0.40    \\ 
% API2      & \multicolumn{1}{c|}{0.64}   & 0.38    & \multicolumn{1}{c|}{0.64}   & 0.39    & \multicolumn{1}{c|}{0.65}   & 0.40    \\ 
% API3      & \multicolumn{1}{c|}{\textbf{0.65}}   & 0.39    & \multicolumn{1}{c|}{0.65}   & 0.39    & \multicolumn{1}{c|}{0.65}   & 0.40    \\ 
% \midrule
% Var+API & \multicolumn{1}{c|}{0.64}   & 0.39    & \multicolumn{1}{c|}{\textbf{0.66}}   & 0.39    & \multicolumn{1}{c|}{\textbf{0.66}}   & 0.40    \\ 
% \bottomrule
% \end{tabular}
% \label{tab:ablation_k}
% \end{table}
% \subsection{RQ3: Interpreting Models}
% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.48\textwidth]{figures/representation_density_vulnerable_k_1_vs_40.pdf}
% \caption{Prediction Probability Density}
% \label{fig:interpretation-analysis-results}
% \end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.48\textwidth]{figures/representation_density_combined_k_1_vs_40.png}
\caption{Prediction Probability Density of \tool for K=1 and K=40. }
\label{fig:prob_k_1vs40}
\end{figure}

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.48\textwidth]{figures/representation_density_non_vulnerable_k_1_vs_40.pdf}
% \caption{Prediction Probability Density}
% \label{fig:interpretation-analysis-results}
% \end{figure}

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.48\textwidth]{figures/representation_density_non_vulnerable_k_1_vs_40.pdf}
% \caption{Prediction Probability Density}
% \label{fig:interpretation-analysis-results}
% \end{figure}

\begin{table}[]

\caption{The performance of the Causal Approach when different early layer is used.}
\begin{tabular}{l|c|c|c}
\toprule
Model         & Early Layer          & \begin{tabular}[c]{@{}c@{}}Devign\\ (Var+API)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Big-Vul\\(Var+API)\end{tabular} \\
\midrule
CodeBERT      & 1  & 0.6494   & 0.4034   \\
CodeBERT      & 2 & 0.6528  & 0.4018    \\
CodeBERT      & 3                    & 0.6501                                                       & 0.4026                                                    \\
CodeBERT      & 4                    & 0.6546                                                       & 0.4055                                                    \\
\midrule
GraphCodeBERT & 1                    & 0.6156                                                       & 0.3916                                                    \\
GraphCodeBERT & 2                    & 0.6170                                                       & 0.3903                                                    \\
GraphCodeBERT & 3                    & 0.6363                                                       & 0.3908                                                    \\
GraphCodeBERT & 4                    & 0.6570                                                       & 0.3927                                                    \\
\midrule                            
UniXcoder     & 1                    & 0.5728                                                       & 0.4049                                                    \\
UniXcoder     & 2                    & 0.5720                                                       & 0.4055                                                    \\
UniXcoder     & 3                    & 0.5550                                                       & 0.4056                                                    \\
UniXcoder     & 4                    & 0.6609                                                       & 0.4058  \\
\bottomrule
\end{tabular}
\label{tab:ablationel}
\end{table}
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \begin{table}[]
% % \begin{tabular}{|l|cc|cc|cc|}

% % \end{tabular}
% \end{table}
Table \ref{tab:ablationel} demonstrates the result of using different early layers to extract $M$. We choose the {\it Var+API} settings for all models to present the result. Overall, the result shows that layer four performs better than the other three layers. 

==> body/99.TODO_and_Help.tex <==
\section{TODO and Help}
\subsection*{TODOs}
%To write the todos mention the name to who the todo is assigned. See the Help guide for the maros.
\begin{enumerate}
    \item Inference time, how many X' to be selected 
\end{enumerate}

\subsection*{Help}
\begin{itemize}
    \item To write a code in one line, \linecode{public static void main (String args[])}
    \item To write full code (mind the spacing of the code in the latex file),
    
    \lstset{escapechar=@,style=CustomJavaWoNumbers}
\begin{lstlisting}
public static void main (String[] args) {
    System.out.println("Hello world!");
}
\end{lstlisting} 
    \medskip
    \item To highlight something with a box, \\\highlight{This line needs to be highlighted}
    \item For writing any code with error \errorcode{statioc void main}
    \item To highlight a lesson learned, \lessons{lesson learned}
    \item For research questions, see \Cref{sec:experiments} and \Cref{sec:results}.
    \item To leave comment for specific persons,
        \begin{itemize}
            \item \russell{ to assign to Russell}
            \item \ira{to assign to Ira}
            \item \wei{to assign to Wei}
            \item \ray{to assign to Baishakhi}
            \item \saikat{to assign to Saikat}\\
        \end{itemize}
\end{itemize}

==> body/ChengZhiDraft.tex <==
\section{Causal Learning to Remove Spurious Features}
%Background?
%\section{Do Calculus for Vulnerability Detection: Background}
\label{sec:background}

%Chengzhi and Wei

% In this section, we provide the background and also formulate {\it do calculus} for vulnerability detection.

To fundamentally understand the reason of spurious features in code vulnerability detection, we will use our domain knowledge of the code problem  formulate how the program data is generated in causal language, which also allows us to understand why there is distribution shifts in a principled way. We will then derive the signal we need to learn to generalize and robust. We will then study how to calculate the estimand to generalize. 

\subsection{Causal Graph for Vulnerability Detection}
To apply causal learning, our first step is to construct a {\it causal graph} to model the data generation process. In a causal graph, node 

We first formulate the data generation process of code vulnerability using causal graph. We denote the input code as $X$ and the label for code vulnerability as $Y$. We denote the programmer as node $U$, which is latent and not observed in the training data distribution. $U$ denotes the level or coding style of the programmer, it will write the code through first design the basic features of the code $M$, such as coming up with the the name of the code variable, the API to call from the code. The features $M$ will form the code $X$ together with the code specification $C$. $C$ is the specification and function of the project, which might contain vulnerability design not related to specific programmer style, for example, with dealing with pointer in C, there tends to be vulnerability. The code $X$ is constructed with the specification $C$ together with the programmer's variable name and API choice $M$. The level of the programmer will  affects whether the code contains bug of not, for example, junior programmer tends to write code with vulnerability issue, and they tends to name the variable with specific name format $M$, or writing dead API call, thus we draw an arrow from $U$ to $Y$. We use gray node to denote the node that can be observed.

This causal graph will introduce this join distribution of data, which will create the observation data we observe in the training and testing set. If we train the standard deep learning model, using the code $X$ as input, to predict the vulnerability label $Y$, we will learn this correlation $P(Y|X)$. If there is no domain shifts and environment change, i.e., the testing data is i.i.d., the model that use this correlation will generalize perfectly.

\subsection{Modeling Domain Shifts through Causal Transportability}

However, once we train our vulnerablity detection model, we are going to deploy it in the open, real world setting, where the i.i.d. hypothesis often does not hold. 
We will first fundamentally discuss how the distribution will shifts in a principled way.
The domain shifts is introduce by the change of the environment node $E$. At training time, say $E=0$, this environment often employ programmers of junior level. At testing, say $E=1$, this company tends to employ programmer from a senior level. The change of $E$ will introduce the domain shifts in code from training to testing. Note that $E$ can be continuous varaible, here we use binary variable for simplicity. Due to the shifting of $E$ from 0 to 1, the correlation $P(Y|X)$ will be different, because $X$ and $Y$ nodes are both decedent of the $E$ node and will be affect by its change, i.e., $P(Y|X, E=0) \neq P(Y|X, E=1)$. Now we have derived the reason, natural code data will not be i.i.d.. Thus, if we use the typical deep learning models that learn correlation, the learned signal will not generalize and perform bad on new environment.


 % now discuss why correlation based learn
\subsection{Causal Effect Can Generalize across Environments for Code Vulnerability Detection}

To generalize, our goal is to learn the signal that is invariant from training to testing. If we intervene on the causal graph, so that the correlation between $X$ and $Y$ is the same no matter how the environment $E$ change, then we can apply the standard deep learning method to learn correlation, which can automatically generalize to new testing environment. 

As shown in Figure, if we can directly intervene on the code $X$. Instead of samping the code from the original joint distribution of the code generation, imagine we can ask an oracle to write perfect, unbiased code for us, and use those code to replace the original code $X$. Now, for this new causal graph, we will remove all the incoming edges to node $X$, and put our own new code $x$ here $X=x$. In this new causal graph, since the node $E$ is not impacting both $X$ and $Y$, the correlation between $X$ and $Y$ will be the same despite the change of $X$. We have $P(Y|X, E=0) = P(Y|X, E=1)$ in the new interventional causal graph. This is the invariant signal we need to generalize from training to testing. In the literature, this correlation under this new intervention causal graph, is defined as the causal effect from code to vulerability label, which people denotes as $P(Y|Do(X=x))$.

Now we have derived that, to generalize robustly to new environment and distribution shifts in code vulenrability detection, we need to learn the causal effect of $P(Y|Do(X))$.


\subsection{Identifying Causality through Observational Data}

Since it is infeasible to actually have the oracle that writes the perfect, unbiased code for us at scale, we will investigate how to learn the causal effect from our given observational data. With our domain knowledge, we can estimate the value for the latent spurious features, $M$. We now can derive the causal effect without actually perform the intervention following the backdoor criteria:

\begin{equation}
    P(Y|Do(X)) = \sum_{M'_1, M'_2} P(Y|X, M'_1, M'_2) P(M'_1)P(M'_2)
\end{equation}

Intuitively, once we condition on the intermediate features $M$, there will be no direct information flow from $E$ to $X$, thus the change of the environment $E$
will not simultaneously affect $X$ and $Y$, which will not introduce any spurious correlation. To calculate the above estimand, we need to randomly sample feature $M$ from random code, and feed them into the equation.

From a code perspective, the original code data $X$ contains both core features for vulnerability and the spurious features for vulnerability.Spurious features are $M$ features, which will subject to change once the environment or programmer style change. By first learning to predict $Y$ from both $M$ and $X$, the model will learn to use the spurious features $M$ in the $M$ input branch. Since by condition on $M$, the spurious features in code is no longer informative to predict $Y$, thus for the model input branch that takes in $X$, it will mostl learn the core, robust features that are not related to programmer style. 

At inference, we will remove the effect of the spurious features $M$ by averaging it over random sampled $M$, which makes  $M$ feature not contributing to the final prediction. Thus, this new estimand can only use the core, robust features to make the right prediction, despite the change of the environment $E$.

======



Learn casual effects, we need to perform {\it do} calculus. Intervention that estimate the probability based on only cause $C$ of the vulnerability  

$P(Y|X)$ = causal + spurious 

$P*(Y|X)$ = causal + spurious*

$P(Y|X)\neq P*(Y|X)$ 

$P(Y|do(X)) = P*(Y|do(X))$ \wei{should we use C or X here}

$P(Y|do(X))$ use causal features only to predict Y

Difference:
Here, we assume that not all the back door variables are observable 

\subsection{Causal Diagram and Backdoor Variables}
Applying causal inference, we first construct casual structure to model the vulnerability detection

\wei{is this diagram correct?}

\begin{figure}[htb]
\centering
\includegraphics[width=0.3\textwidth]{figures/icse2.jpeg}
\caption{Causal Structure of Vulnerability Detection}
\label{fig:causalstructure}
\end{figure}

\subsection{Computing Do Calculus: the Math Formula and the Assumptions}

Formula 1 in~\cite{2022cvprmao}

How to perform do calculus? The assumptions of our approaches

Assumption 1~\cite{2022cvprmao} applies here:
X = W (spurious) +Z (causal);
R = W (spurious) +Z (causal)

W are not confounding with Z, as the two have no direct relations?

Assumption 2~\cite{2022cvprmao} is a strong assumption, but we still assume: representation captures the causal features 

{\it require a strong model that can learn the best representation}

Assumption 3~\cite{2022cvprmao}


Step 1: build a model that uses both spurious and causal features to predict

Step 2: during inference, only can use causal features 


\section{Algorithm}
% Rasel 

% If we follow the backdoor, we can talk less about the assmption, and not follow the same one as CVPR Mao.



The components: $P(R|X)$ -- Assumption 2
We are using the STOA models to learn a source code representation

$\hat{P}(Y|R,X')$ -- Assumption 3

X' should encode S1-Sn token level (Variable name, API names) features

Phrase 1: learn the causal as well as the spurious features

find an example that can expose spurious feature

Phrase 2:  marginalizing over the spurious features, discard the spurious models 

\begin{itemize}
    \item name swap: select the example with similar names 
\end{itemize}


%\subsection{Put together: The Algorithm}

Modify algorithms to emphasize our novel part
